Estimation Contracts for Outlier-Robust Geometric Perception

Outlier-robust estimation is a fundamental problem and has been extensively investigated by statisticians and practitioners. The last few years have seen a convergence across research fields towards "algorithmic robust statistics", which focuses on developing tractable outlier-robust techniques for high-dimensional estimation problems. Despite this convergence, research efforts across fields have been mostly disconnected from one another. This monograph bridges recent work on certifiable outlier-robust estimation for geometric perception in robotics and computer vision with parallel work in robust statistics. In particular, we adapt and extend recent results on robust linear regression (applicable to the low-outlier regime with << 50% outliers) and list-decodable regression (applicable to the high-outlier regime with >> 50% outliers) to the setup commonly found in robotics and vision, where (i) variables (e.g., rotations, poses) belong to a non-convex domain, (ii) measurements are vector-valued, and (iii) the number of outliers is not known a priori. The emphasis here is on performance guarantees: rather than proposing radically new algorithms, we provide conditions on the input measurements under which modern estimation algorithms (possibly after small modifications) are guaranteed to recover an estimate close to the ground truth in the presence of outliers. These conditions are what we call an "estimation contract". Besides the proposed extensions of existing results, we believe the main contributions of this monograph are (i) to unify parallel research lines by pointing out commonalities and differences, (ii) to introduce advanced material (e.g., sum-of-squares proofs) in an accessible and self-contained presentation for the practitioner, and (iii) to point out a few immediate opportunities and open questions in outlier-robust geometric perception.

==> app-certifiable-anti-con.tex <==
%!TEX root = main.tex

\section{Certifiable Anti-Concentration}
\label{app:certifiable-anti-con}

Let matrix have certifiable anti-concentrated columns.
 Then, matrix is $d$ certifiably anti-concentrated.

 Apply definition component-wise:
\begin{align}
&\forall \vv \;, \; \normTwo{\va_j\tran \vv}^2 
\leq \delta^2 \Expect{}{ \normTwo{\va_j\tran \vv}^2 }  \quad \text{implies} \quad
\left( {p_j\left(\va_j\tran \vv \right)} -1 \right)^2\leq \delta^2 \label{eq:certAntiCon1_app}
\\
&\forall \vv \;, \; \toAsk{\normTwo{\vv}^2 \leq 1} \quad \text{implies} \quad
\Expect{}{ p_j^2\left(\va_j\tran \vv \right) } \leq C \, \delta \label{eq:certAntiCon2_app}
\end{align}

Summing all of them (recall fact).

Now recall that 


\begin{align}
&\forall \vv \;, \;  \sumOverDimy \normTwo{\va_j\tran \vv}^2 
\leq \delta^2 \sumOverDimy \Expect{}{ \normTwo{\va_j\tran \vv}^2 }  \quad \text{implies} \quad
\left( {p_j\left(\va_j\tran \vv \right)} -1 \right)^2\leq \delta^2 
\\
&\forall \vv \;, \; \toAsk{\normTwo{\vv}^2 \leq 1} \quad \text{implies} \quad
\Expect{}{ p_j^2\left(\va_j\tran \vv \right) } \leq C \, \delta 
\end{align}

==> app-proof-lowOut-apriori-LTS-noiseless.tex <==
%!TEX root = main.tex

\section{Proof of Theorem~\ref{thm:lowOut-apriori-LTS} (noiseless)}
\label{app:proof-lowOut-apriori-LTS}

We start by restating the theorem for the reader's convenience.

\noindent\fbox{
\parbox{\textwidth}{
\begin{theorem}[Restatement of Theorem~\ref{thm:lowOut-apriori-LTS}]
\ltsThm
\end{theorem}
}}

Before proving the theorem we need to prove two technical lemmas that we present in~\cref{eq:boundxxgt}
 and~\cref{lem:exists_vi} below. These lemmas extend results~\cite{Karmalkar19neurips-ListDecodableRegression} 
 to vector-valued measurements, and while in~\cite{Karmalkar19neurips-ListDecodableRegression}  they have been proposed to attack the high-outlier case (\ie for list-decodable regression), we show they are also useful to 
 prove estimation contracts for the low-outlier case.
 
 Note that the two lemmas below use a larger constraint set compared to the one in~\eqref{eq:LTS-T} (\ie which does not contain the constraint $\sumOverMeas{\omega_i} = \alpha \nrMeasurements$): this will allow to use them also to discuss the performance of~\eqref{eq:MC} and~\eqref{eq:TLS}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Adapted from Lemma 4.1 in~\cite{Karmalkar19neurips-ListDecodableRegression}]
\label{eq:boundxxgt}
Consider the following constraint set, for given measurements $(\vy_i,\MA_i)$, $i \in [\nrMeasurements]$, 
a constant $\barc \geq 0$, and where $\Domain$ is a basic semi-algebraic set: \LC{explicitly bounded}
\begin{align}
\axiomsMC \doteq \left\{
    \begin{array}{cl}
    \omega_i^2 = \omega_i, \;\; i\in[\nrMeasurements] \\ 
    \omega_i \cdot \residuali{\vxx}^2 \leq \barc^2 \;\; i\in[\nrMeasurements]\\
    \vxx \in \Domain
    \end{array}
    \right\}
\end{align}

For any $t \geq k$ and set of $\nrMeasurements$ measurements with at least $\an$ inliers, such that for the set of inliers $\setInliers$ the set of matrices $\MA_i$, $i\in\setInliers$ is
$k$-certifiably $(C,\frac{\inlierRate^2 \eta^2}{4C})$-anti-concentrated,
\begin{align}
\axiomsMC \sosimply{\vomega,\vxx}{t}
\left\{
\aveOverInliers \omega_i \normTwo{\vxx - \vxx\gt}^2 \leq \frac{\inlierRate^2 \eta^2 \boundx^2}{2}
\right\}.
\end{align}
\end{lemma}

\begin{proof} % lemma
% \grayout{ We start by observing that since $\normTwo{\vxx} \leq \boundx$, then $\axiomsMC\sosimply{\vxx}{t} \normTwo{\vxx - \vxx\gt}^2 \leq 2 \boundx^2$. }
Since the set of matrices $\MA_i$, $i\in\setInliers$, is $(C,\frac{\inlierRate^2 \eta^2}{4C})$-anti-concentrated, then there exists
 a univariate polynomial $p$ such that for every $i \in [\nrMeasurements]$:
 \begin{align}
 \label{eq:proof21}
\overbrace{
\left\{ \omega_i \cdot \normTwo{\MA_i\tran (\vxx-\vxx\gt)}^2 = 0 \right\} 
\sosimply{\vxx}{t} 
\left\{ p\left(\omega_i \cdot \normTwo{\MA_i\tran (\vxx-\vxx\gt)}^2 \right) = 1 \right\}
}^{ \text{using \eqref{eq:certAntiConSet1} with $\delta=0$} }
 \end{align}
 and
 \begin{align}
 \label{eq:proof22}
\normTwo{\vxx}^2 \leq \boundx
 \overbrace{
\sosimply{\vxx}{t} \normTwo{\vxx - \vxx\gt}^2 \leq 2 \boundx^2
}^{\text{using the triangle inequality~\eqref{eq:sosTriangleNorm} }}
 \overbrace{
\sosimply{\vxx}{t} 
\left\{ \aveOverInliers p^2\left(\normTwo{\MA_i\tran (\vxx-\vxx\gt)}^2 \right) \leq \frac{\inlierRate^2\eta^2}{4} \right\}
}^{\text{using anti-concentration in eq.~\eqref{eq:certAntiConSet2} }}
\end{align}

Using~\eqref{eq:proof21}: 
\begin{align}
\axiomsMC
\overbrace{
\sosimply{\vomega,\vxx}{ \red{2t} }
\left\{
1-p^2(\omega_i \cdot \normTwo{\MA_i\tran (\vxx-\vxx\gt)}^2) =0 
\right\}
}^{\text{ {squaring both members} in~\eqref{eq:proof21} and using~\cref{fact:sossquaring}}}
\\
\overbrace{
\sosimply{\vomega,\vxx}{2t}
\left\{
1-\omega_i p^2\left( \normTwo{\MA_i\tran (\vxx-\vxx\gt)}^2 \right) =0 
\right\}
}^{\text{since $\omega_i$ is binary and $p(0)=1$}}
\label{eq:proof41}
\end{align}
%
Using~\eqref{eq:proof22} and $\axiomsMC
\sosimply{\vomega}{2} \{\omega_i^2 = \omega_i\}$, we obtain:
\begin{align}
\axiomsMC
\sosimply{\vomega,\vxx}{t+2}
\Big\{
\aveOverInliers \omega_i \normTwo{\vxx-\vxx\gt}^2 
\overbrace{
= \aveOverInliers \omega_i \normTwo{\vxx-\vxx\gt}^2 \cdot \omega_i  p^2\left( \normTwo{\MA_i\tran (\vxx-\vxx\gt)}^2 \right)
}^{\text{ since $\omega_i p^2\left( \normTwo{\MA_i\tran (\vxx-\vxx\gt)}^2 \right)=1$ per~\eqref{eq:proof41} }}
\\ 
\overbrace{
= \aveOverInliers \omega_i \normTwo{\vxx-\vxx\gt}^2 \cdot p^2\left( \normTwo{\MA_i\tran (\vxx-\vxx\gt)}^2 \right)
}^{\text{using $\omega_i^2 = \omega_i$ in $\axiomsMC$}}
\\
\overbrace{
\leq \aveOverInliers \red{\normTwo{\vxx-\vxx\gt}^2} \cdot p^2\left( \normTwo{\MA_i\tran (\vxx-\vxx\gt)} \right)
}^{\text{upper-bound when all $\omega_i=1$}}
\overbrace{
 \leq \frac{\inlierRate^2 \eta^2 \boundx^2}{2}
 }^{\text{using~\eqref{eq:proof22}}}
 \Big\}
\end{align}
concluding the proof.
\end{proof} % lemma

% As a consequence, we can show below that a constant fraction of suitable vectors built from the pseudo-moment 
% matrix satisfying constraints  are close to $\vxx\gt$.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Adapted from Lemma 4.2 in~\cite{Karmalkar19neurips-ListDecodableRegression}] \label{lem:exists_vi}
Under the same assumptions of~\cref{eq:boundxxgt}, 
for any $\pdist$ of degree $k$ satisfying $\axiomsMC$,
\begin{align} 
\aveOverInliers \pExpect{\pdist}{\omega_i} \normTwo{\vv_i-\vxx\gt} \leq \frac{\inlierRate \eta \boundx}{\sqrt{2}},
\end{align}
where the vectors $\vv_i$ are extracted from the pseudo-moment matrix by setting $\vv_i = \frac{\pExpect{\pdist}{\omega_i\vxx}}{\pExpect{\pdist}{\omega_i}}$ if $\pExpect{\pdist}{\omega_i} > 0$, or $\vv_i = \zero$ otherwise, for $i\in[\nrMeasurements]$.
%   $\vv_i$ are extracted from the pseudo-moment matrix via $\vv_i \triangleq 
% \frac{\pExpect{\pdist}{\vxx \; \omega_i}}{ \pExpect{\pdist}{\omega_i} }$, $i\in[\nrMeasurements]$.
\end{lemma}
\begin{proof}% lemma
By~\cref{eq:boundxxgt}, we have $\axiomsMC\sosimply{\vomega,\vxx}{k}
\left\{
\aveOverInliers \omega_i \normTwo{\vxx - \vxx\gt}^2 \leq \frac{\inlierRate^2 \eta^2 \boundx^2}{2}
\right\}$.
We also have: $\axiomsMC
\sosimply{\vomega}{2} \{\omega_i^2 = \omega_i\}$ for any $i$. Therefore:
\begin{align}
\axiomsMC\sosimply{\vomega,\vxx}{k}
\left\{
\aveOverInliers \normTwo{ \omega_i\vxx -  \omega_i \vxx\gt}^2 \leq \frac{\inlierRate^2 \eta^2 \boundx^2}{2}
\right\}
\end{align}
Since $\pdist$ satisfies $\axiomsMC$, then it also satisfies:
\begin{align}
\aveOverInliers \pExpect{\pdist}{  
\normTwo{ \omega_i\vxx -  \omega_i \vxx\gt}^2} 
\leq \frac{\inlierRate^2 \eta^2 \boundx^2}{2}
\label{eq:proof51}
\end{align}
\red{Using Jensen's inequality} $\normTwo{ \pExpect{\pdist}{\omega_i\vxx -  \omega_i \vxx\gt}}^2  \leq \pExpect{\pdist}{  
\normTwo{ \omega_i\vxx -  \omega_i \vxx\gt}^2}$; then using \CS for pseudo-distributions (\cref{fact:CSforpdist}) on $\normTwo{ \pExpect{\pdist}{\omega_i\vxx -  \omega_i \vxx\gt}}^2$ and chaining the inequalities back to~\eqref{eq:proof51}:
\begin{align}
\left( 
\aveOverInliers   
\normTwo{ \pExpect{\pdist}{ \omega_i\vxx } -  \pExpect{\pdist}{ \omega_i } \vxx\gt }
\right)^2
\\
\overbrace{\leq}^{\text{using~\cref{fact:CSforpdist}}} 
\aveOverInliers 
\normTwo{ \pExpect{\pdist}{ \omega_i\vxx } -  \pExpect{\pdist}{ \omega_i } \vxx\gt }^2
 \leq \frac{\inlierRate^2 \eta^2 \boundx^2}{2}
\end{align}
Remembering that  $\vv_i = \frac{\pExpect{\pdist}{\omega_i\vxx}}{\pExpect{\pdist}{\omega_i}}$ if $\pExpect{\pdist}{\omega_i} > 0$, or $\vv_i = \zero$ otherwise, we have
\begin{align}
\frac{1}{\setInliers} \sum_{i \in |\setInliers|, \pExpect{\pdist}{\omega_i} > 0} 
\pExpect{\pdist}{\omega_i}^2 \normTwo{\vv_i - \vxx\gt}^2
 \leq \frac{\inlierRate^2 \eta^2 \boundx^2}{2}\label{eq:proof52}
\end{align}
\red{Using Jensen's inequality again:}
\begin{align}\left( \frac{1}{\setInliers} \sum_{i \in |\setInliers|, \pExpect{\pdist}{\omega_i} > 0} 
\pExpect{\pdist}{\omega_i} \normTwo{\vv_i - \vxx\gt} \right)^2
 \leq \frac{1}{\setInliers} \sum_{i \in |\setInliers|, \pExpect{\pdist}{\omega_i} > 0} 
\pExpect{\pdist}{\omega_i}^2 \normTwo{\vv_i - \vxx\gt}^2 \label{eq:proof53}
\end{align} 
Chaining~\eqref{eq:proof52} and~\eqref{eq:proof53} and 
taking the square root of both members we finally prove the claim:
\begin{align}
\frac{1}{\setInliers} \sum_{i \in |\setInliers|, \pExpect{\pdist}{\omega_i} > 0} 
\pExpect{\pdist}{\omega_i} \normTwo{\vv_i - \vxx\gt}
 \leq \frac{\inlierRate \eta \boundx}{\sqrt{2}}.
\end{align}
\end{proof}% lemma


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof of Theorem~\ref{thm:lowOut-apriori-LTS}:]
First of all, we note that since $\axiomsLTST$ contains a superset of the constraints in $\axiomsMC$ defined in~\cref{eq:boundxxgt}, the conclusions of~\cref{lem:exists_vi} and~\cref{eq:boundxxgt} still hold if we replace $\axiomsMC$ with $\axiomsLTST$.
 Therefore we have that any pseudo-distribution satisfying $\axiomsLTST$ also satisfies:
\begin{align}
\label{eq:boundInliers}
\aveOverInliers \pExpect{\pdist}{\omega_i} \normTwo{\vv_i-\vxx\gt} \leq \frac{\inlierRate \eta \boundx}{\sqrt{2}}
\iff 
\sumOverInliers \pExpect{\pdist}{\omega_i} \normTwo{\vv_i-\vxx\gt} \leq \frac{\inlierRate \eta \boundx}{\sqrt{2}}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Now we observe that since $\pExpect{\pdist}{\omega_i} \leq 1$, then 
$\sumOverOutliers \pExpect{\pdist}{\omega_i} \leq (1-\inlierRate)\nrMeasurements$.
Moreover, recalling that $\normTwo{\vv_i-\vxx\gt} \leq \sqrt{2} \boundx$:
\begin{align}
\label{eq:boundOutliers}
\sumOverOutliers \pExpect{\pdist}{\omega_i} \normTwo{\vv_i-\vxx\gt}  \leq \nrMeasurements  \sqrt{2} \boundx (1-\inlierRate)
\end{align}

Using~\cref{eq:boundInliers} and~\cref{eq:boundOutliers}:
\begin{align}
\sumOverMeas \pExpect{\pdist}{\omega_i} \normTwo{\vv_i-\vxx\gt} =  
\sumOverInliers \pExpect{\pdist}{\omega_i} \normTwo{\vv_i-\vxx\gt} 
+ \sumOverOutliers \pExpect{\pdist}{\omega_i} \normTwo{\vv_i-\vxx\gt}
\\
 \leq \frac{\inlierRate^2 \; \eta \; \boundx \; \nrMeasurements}{\sqrt{2}} + \nrMeasurements  \sqrt{2} \boundx (1-\inlierRate)
\end{align}
%
Now note that \LC{need bound on $\sumOverMeas \pExpect{\pdist}{\omega_i}$}
Dividing both members by $\sumOverMeas \pExpect{\pdist}{\omega_i}$:
\begin{align}
\label{eq:proof61}
\sumOverMeas \frac{ \pExpect{\pdist}{\omega_i} }{ \sumOverMeas \pExpect{\pdist}{\omega_i} } \normTwo{\vv_i-\vxx\gt} 
 \leq \frac{1}{\sumOverMeas \pExpect{\pdist}{\omega_i} }
 \left( 
 \frac{\inlierRate^2 \; \eta \; \boundx \; \nrMeasurements}{\sqrt{2}} + \nrMeasurements  \sqrt{2} \boundx (1-\inlierRate)
 \right)
 \\
  \leq 
 \frac{1}{\an } \left( 
\frac{\inlierRate^2 \; \eta \; \boundx \; \nrMeasurements}{\sqrt{2}} + \nrMeasurements  \sqrt{2} \boundx (1-\inlierRate)
 \right)
\end{align}
Using Jensen's inequality $\normTwo{ \sumOverMeas \frac{ \pExpect{\pdist}{\omega_i} }{ \sumOverMeas \pExpect{\pdist}{\omega_i} } \vv_i  - \vxx\gt} \leq \sumOverMeas \frac{ \pExpect{\pdist}{\omega_i} }{ \sumOverMeas \pExpect{\pdist}{\omega_i} } \normTwo{\vv_i-\vxx\gt}$ hence~\eqref{eq:proof61} becomes: 
\begin{align}
\normTwo{ \sumOverMeas \frac{ \pExpect{\pdist}{\omega_i} }{ \sumOverMeas \pExpect{\pdist}{\omega_i} } \vv_i  - \vxx\gt} 
\leq
 \frac{\inlierRate \; \eta \; \boundx }{\sqrt{2}} +  \sqrt{2} \boundx \frac{1-\inlierRate}{\inlierRate}
\end{align}
which, recalling that $\vxx\ltssdpT = \sumOverMeas \frac{ \pExpect{\pdist}{\omega_i} }{ \sumOverMeas \pExpect{\pdist}{\omega_i} } \vv_i$, concludes the proof.

\end{proof}

==> discarded-preliminaries.tex <==
%!TEX root = main.tex

\subsection{Semidefinite Programming}

The feasible set of \eqref{eq:primalSDP}, denoted by $\setsdpp\!\triangleq\!\{\!\MX\!\in\!\bbX\!\mid\!\calA(\MX)\!=\!\vb,\MX\!\in\!\calK\}$, \mbox{is called a \emph{spectrahedron} \cite{Blekherman12Book-sdpandConvexAlgebraicGeometry}.} 

The Lagrangian \emph{dual} of \eqref{eq:primalSDP} is another multi-block SDP:
\begin{equation}\label{eq:dualSDP}
\max_{\vy \in \Real{m}, \MS \in \bbX} \cbrace{\inprod{\vb}{\vy} \mid \calAadj(\vy) + \MS = \MC,\ \MS \in \calK} \tag{D}
\end{equation}
where $\calAadj: \Real{m} \rightarrow \bbX$ is the adjoint of $\calA$ and is defined as:
\beq \label{eq:adjointAmultiblk}
\calAadj(\vy) \triangleq \left( \sum_{j=1}^m y_j \MA_{1j},\dots,\sum_{j=1}^m y_j \MA_{lj} \right) \in \bbX
\eeq
and the equality $\calAadj(\vy) + \MS = \MC$ is enforced block-wise.
 % $\calAadj(\vy) \triangleq ( \calAadj_1(\vy),\dots,\calAadj_l(\vy) ) $ for any $\vy \in \Real{m}$, where $\calAadj_i: \Real{m} \rightarrow \sym{n_i}$ defines the $i$-th adjoint map $\calAadj_i(\vy) = \sum_{j=1}^m y_j \MA_{ij}$, 

% $\bbX \triangleq \sym{n_1} \times \dots \times \sym{n_l}, n_1\geq \dots \geq n_l$ is the domain of $\MX = (\MX_1,\dots,\MX_l)$, $\calK \triangleq \psd{n_1} \times \dots \times \psd{n_l}$ is a product of $l$ positive semidefinite cones (blocks), $\MC = (\MC_1,\dots,\MC_l) \in \bbX$ defines a \emph{linear} objective $\inprod{\MC}{\MX} \triangleq \sum_{i=1}^l \inprod{\MC_i}{\MX_i}$, $\vb \in \Real{m}$, and $\calA: \bbX \rightarrow \Real{m}$ is a linear map defined as $\calA (\MX) \triangleq \sum_{i=1}^l \calA_i (\MX_i)$, where $\calA_i: \sym{n_i} \rightarrow \Real{m}$ defines the $i$-th linear map $\calA_i (\MX_i) \triangleq [\inprod{\MA_{ij}}{\MX_i}]_{j=1}^m$ with $\MA_{ij} \in \sym{n_i},j=1,\dots,m$. The feasible set of \eqref{eq:primalSDP}, denoted by $\setsdpp \triangleq \{\MX \in \bbX \mid \calA(\MX)=\vb,\MX \in \calK \}$, is called a \emph{spectrahedron} \cite{Blekherman12book-SDP}. Let $\calAadj: \Real{m} \rightarrow \bbX$ be the adjoint of $\calA$ defined as $\calAadj(\vy) \triangleq ( \calAadj_1(\vy),\dots,\calAadj_l(\vy) ) $ for any $\vy \in \Real{m}$, where $\calAadj_i: \Real{m} \rightarrow \sym{n_i}$ defines the $i$-th adjoint map $\calAadj_i(\vy) = \sum_{j=1}^m y_j \MA_{ij}$, the Lagrangian \emph{dual} of \eqref{eq:primalSDP} reads

Under mild assumptions (\eg Slater's condition \cite{Boyd04book}), \emph{strong duality} holds between \eqref{eq:primalSDP} and \eqref{eq:dualSDP} (\ie the minimum of \eqref{eq:primalSDP} equals the maximum of \eqref{eq:dualSDP}). In this case, $(\MXstar,\vystar,\MSstar) \in \bbX \times \Real{m} \times \bbX$ is simultaneously \emph{optimal} for \eqref{eq:primalSDP}-\eqref{eq:dualSDP} if and only if the following KKT conditions hold
% \begin{subequations}
\beal\label{eq:sdpKKT}
\text{\grayout{primal feasibility}}: & \calA(\MXstar) = \vb, \MXstar \in \calK, \\
\text{\grayout{dual feasibility}}: & \calAadj(\vystar) + \MSstar = \MC, \MSstar \in \calK, \\
\text{\grayout{complementarity}}: & \inprod{\MXstar}{\MSstar} = 0.
\eeal
The KKT conditions \eqref{eq:sdpKKT} imply strong duality because
\begin{equation}
\begin{split}
0 & = \inprod{\MXstar}{\MSstar} = \inprod{\MXstar}{\MC - \calAadj(\vystar)} \\
& = \inprod{\MC}{\MXstar} - \inprod{\calA(\MXstar)}{\vystar}  = \inprod{\MC}{\MXstar} - \inprod{\vb}{\vystar} .
\end{split}
\end{equation}
% \end{subequations}
Given $(\MX,\vy,\MS) \in \calK \times \Real{m} \times \calK$, we measure its feasibility and optimality using the standard relative KKT residuals
% \begin{subequations}
\beal\label{eq:KKTresiduals}
\pfeas  \triangleq & \Vert \calA(\MX) - \vb \Vert  / ( 1+\norm{\vb}), \\
\dfeas  \triangleq &  \Vert {\calAadj(\vy) + \MS - \MC} \Vert  / ( 1+\norm{\MC} ),\\
\gap \triangleq & \abs{\inprod{\MC}{\MX} - \inprod{\vb}{\vy} } / ( 1 +  \abs{ \inprod{\MC}{\MX} } + \abs{ \inprod{\vb}{\vy} } ),
\eeal
% \end{subequations}
where $\norm{\MX} = \sum_{i=1}^l \norm{\MX_i}$ for any $\MX \in \bbX$. We define $\kkt \triangleq \max\{\pfeas,\dfeas,\gap \}$ as the \emph{maximum KKT residual}.

==> highOut-aPosterioriResults.tex <==
%!TEX root = main.tex

\subsection{A Posteriori Estimation Contracts}
\label{sec:highOut-aPosterioriResults}

Tautology: 

\begin{fact}[MC High-Outlier Case: A-Posteriori Estimation Contract]\label{thm:highOut-aposterioriNoisyMC}
no subset of $d$ outliers satisfies the constraints + some conditions on inliers 
\end{fact}


\begin{fact}[TLS High-Outlier Case: A-Posteriori Estimation Contract]\label{thm:highOut-aposterioriNoisyTLS}
no subset of outliers achieves smaller cost + some conditions on inliers
\end{fact}



==> highOut-aPrioriResults-LDR-closestToKarma.tex <==
%!TEX root = main.tex

\subsection{A Priori Estimation Contracts}
\label{sec:highOut-aPrioriResults}

adversary can corrupt more than $50\%$ of the measurements.

idea: return a list of potential candidates. Estimating the variable with a single estimate is information-theoretically impossible. 
goal: output a small (of size only depending on the number of inliers) list

discussion based on~\cite{Karmalkar19neurips-ListDecodableRegression}, but similar result is also presented in
~\cite{Raghavendra20soda-ListDecodableRegressions}.

$\omega_i = 1$ for the measurements selected as inliers and $\omega_i = 0$ for outliers.
Problem below would have multiple solutions, all attaining objective $\sqrt{\inlierRate \nrMeasurements}$.

Key idea:
- soluble: subset such that noise is within bound.
- we can return all subsets of size $\inlierRate \nrMeasurements$ that are soluble. Issue~\cite{Karmalkar19neurips-ListDecodableRegression} number of such subsets is exponential in the dimension of $\vxx$.
- second idea would be to search for disjoint subsets of $[\nrMeasurements]$: this would easily miss good solutions~\cite{Karmalkar19neurips-ListDecodableRegression} 

\begin{align}
\min_{\vomega,\vxx} & \normTwo{\vomega} \\
\subject \axiomsLDR \doteq& \left\{
\begin{array}{cl}
\omega_i^2 = \omega_i, \;\; i=[\nrMeasurements] \\ 
\vxx \in \Domain \\
\sumOverMeas{\omega_i} = \inlierRate \nrMeasurements  \\
\omega_i \cdot \residuali{\vxx} \leq \noiseBound, \;\; i=[\nrMeasurements]
\end{array}
\right\}
\end{align}

Requires stronger assumption compared to hypercontractivity.

\begin{definition}[Anti-Concentration~\cite{Karmalkar19neurips-ListDecodableRegression}]
\label{def:Anticon}
A zero-mean random variable $\vz \in \Real{d}$ has a \emph{$\delta$-anti-concentrated} distribution if 
$\prob{ \vz\tran \vxx = 0  }$ for all non-zero $\vv$. 
A set of vectors $\calZ$ is \emph{$\delta$-anti-concentrated} if the uniform distribution over $\calZ$ is 
$\delta$-anti-concentrated.
\end{definition}

shown to be necessary and sufficient for list-decodable linear regression in~\cite{Karmalkar19neurips-ListDecodableRegression}

intuitively: prevents that set of outliers steals a large set of inliers (\LC{connects to degeneracy?})
 while leading to an estimate that is far from truth.

\grayout{
\LC{following resembles my non-degeneracy condition, not sure if needed}
 \begin{proposition}[Proposition 2.2 in~\cite{Karmalkar19neurips-ListDecodableRegression}]
Suppose $\DistInliers$ is $\inlierRate$-anti-concentrated. 
Suppose there exists a partition $\calS_1,\calS_2,\ldots,\calS_k \subseteq [\nrMeasurements]$ 
such that each $|\calS_i| \geq \inlierRate \nrMeasurements$ and call $\vxx_1,\vxx_2,\ldots,\vxx_k$ 
the corresponding estimates. There for some $i$, $\normTwo{\vxx_i - \vxx\gt} \leq \red{\eta}$. (\LC{Karma does noiseless})
\end{proposition}
}

previous relation essentially says that under anti-concentration assumptions, if we can find a partition 
of $[\nrMeasurements]$ such that each partition is sufficiently large, then we solved the problem.
Prevents estimate from hiding ..

issue: such partition might not exist. 

\begin{definition}[Certifiable Anti-Concentration~\cite{Karmalkar19neurips-ListDecodableRegression}]
\label{def:certAnticon}
A random variable $\vz$ has a \emph{$k$-certifiably $(C,\delta)$-anti-concentrated} distribution if there 
is a univariate polynomial $p$ satisfying $p(0)=1$ such that there is a degree $k$ sum-of-squares proof of the following two inequalities:
\begin{align}
&\forall \vv \;, \; (\vv\tran \vz)^2 \leq \delta^2 \Expect{}{\vv\tran \vz}^2 \quad \text{implies} \quad
\left( p(\vv\tran \vz) -1 \right)^2\leq \delta^2 \label{eq:certAntiCon1}
\\
&\forall \vv \;, \; \normTwo{\vv}^2 \leq 1 \quad \text{implies} \quad
\Expect{}{ p^2(\vv\tran \vz) } \leq C\delta \label{eq:certAntiCon2}
\end{align}
\end{definition}

\begin{algorithm}[h!]
	\caption{List-Decodable Regression~\cite{Karmalkar19neurips-ListDecodableRegression}.\label{algo:ldr}}
	\SetAlgoLined
	\KwIn{ inputs }
	\KwOut{ outputs. }
	solve convex relaxation 
    
    for each $i \in [\nrMeasurements]$ such that $\pExpect{\pdist}{\omega_i} > 0$ let $\vv_i = \frac{\pExpect{\pdist}{\omega_i\vxx}}{\pExpect{\pdist}{\omega_i}}$, or set $\vv_i = \zero$ otherwise.

    sample $O(1/\inlierRate)$ from $[\nrMeasurements]$ with probability $\frac{\pExpect{\pdist}{\omega_i}}{\an}$ and for each extracted $i$ add $\vv_i$ to list $\List$.
    % \For{ a}{
    % 		a
    % 	}

	\Return{$\List$.}
\end{algorithm}

essentially bound probability that high-dimensional random variable has zero projections in any directions.
Anti-concentration inequality are well studied, see, \eg~\cite{Tao12combinatorica}

\noindent\fbox{
\parbox{\textwidth}{
\begin{theorem}[High-Outlier Case: Estimation Contract, adapted from  Theorem 1.5 in~\cite{Karmalkar19neurips-ListDecodableRegression}]
\label{thm:highOut-apriori}
Let $\DistInliers$ be the (inlier) distribution on $\Real{\dimAmbient} \times \Real{\dimy}$, 
such that the marginal on $\Real{\dimAmbient}$ is k-certifiably $(C, \frac{\inlierRate^2 \eta^2}{10C})$-certifiably anticoncentrated distribution for some $\inlierRate > 0$ and $\eta > 0$. 
\red{Assume the inlier noise has variance $\noiseStd^2$.}
For some outlier rate $\outlierRate = (1-\inlierRate)$, consider a $\outlierRate$-corrupted sample with $\nrMeasurements \approx (\dimAmbient \cdot k)^{O(k)}$ measurements, where the inliers are drawn from $\DistInliers$.
Then, with probability at least $0.99$ (over the draw of the samples), (the polynomial-time) Algorithm~\ref{algo:ldr} outputs a list 
$\List$ of size $O(1/\inlierRate)$ such that there is an $\vxx \in \List$ such that 
$\normTwo{\vxx - \vxx\gt} \leq \frac{\noiseStd}{\inlierRate} +  \eta$.
\end{theorem}
}}

impractical: for Gaussians, $k=..$ (\LC{check size of relaxation})

\begin{proof}
We start by proving the following lemma, that states that any $\vxx$ that there is an \sos proof that 
any $\vxx$ that satisfies $\axiomsLDR$ must be ``close'' to the ground truth $\vxx\gt$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Lemma 4.1 in~\cite{Karmalkar19neurips-ListDecodableRegression}]
\label{eq:boundxxgt}
For any $t \geq k$ and set of $\nrMeasurements$ measurements with at least $\an$ inliers, such that the set of inliers $\setInliers$ is 
$k$-certifiably $(C,\frac{\inlierRate^2 \eta^2}{4C})$-anti-concentrated,
\begin{align}
\axiomsLDR \sosimply{\vomega,\vxx}{t}
\left\{
\aveOverInliers \omega_i \normTwo{\vxx - \vxx\gt}^2 \leq \frac{\inlierRate^2 \eta^2}{4}
\right\}.
\end{align}
\end{lemma}

\begin{proof} % lemma
We start by observing that since $\normTwo{\vxx} \leq M_x$, then $\axiomsLDR \sosimply{\vxx}{t} \normTwo{\vxx - \vxx\gt}^2 \leq 2 M_x^2$.
Since $\setInliers$ is $(C,\frac{\inlierRate^2 \eta^2}{4C})$-anti-concentrated, then there exists
 a univariate polynomial $p$ such that for every $i \in [\nrMeasurements]$:
 \begin{align}
 \label{eq:proof21}
\overbrace{
\left\{ \omega_i \cdot \normTwo{\MA_i\tran (\vxx-\vxx\gt)} = 0 \right\} 
\sosimply{\vxx}{t} 
\left\{ p\left(\omega_i \cdot \normTwo{\MA_i\tran (\vxx-\vxx\gt)} \right) = 1 \right\}
}^{ \text{using~\eqref{eq:certAntiCon1} with $\delta = 0$} }
 \end{align}
 and
 \begin{align}
 \label{eq:proof22}
 \overbrace{
\normTwo{\vxx}^2 \leq M_x
\sosimply{\vxx}{t} 
\left\{ \aveOverInliers p\left(\normTwo{\MA_i\tran (\vxx-\vxx\gt)} \right)^2 \leq \frac{\inlierRate^2\eta^2}{4} \right\}
}^{\red{\text{to check for }M_x}}
\end{align}

Using~\eqref{eq:proof21}: \LC{also unclear}
\begin{align}
\axiomsLDR 
\sosimply{\vomega,\vxx}{t+2}
\left\{
1-p^2(\omega_i \cdot \normTwo{\MA_i\tran (\vxx-\vxx\gt)}) =0 
\right\}
\sosimply{\vomega,\vxx}{t+2}
\left\{
1-\omega_i p^2( \normTwo{\MA_i\tran (\vxx-\vxx\gt)}) =0 
\right\}
\end{align}
Using~\eqref{eq:proof22} and $\axiomsLDR 
\sosimply{\vomega}{2} \{\omega_i^2 = \omega_i\}$, we obtain \LC{unclear}:
\begin{align}
\axiomsLDR 
\sosimply{\vomega,\vxx}{t+2}
\Big\{
\aveOverInliers \omega_i \normTwo{\vxx-\vxx\gt}^2 = 
\aveOverInliers \omega_i \normTwo{\vxx-\vxx\gt}^2 \omega_i p^2( \normTwo{\MA_i\tran (\vxx-\vxx\gt)} )
\\ 
= \aveOverInliers \omega_i \normTwo{\vxx-\vxx\gt}^2 p^2( \normTwo{\MA_i\tran (\vxx-\vxx\gt)} )
\\
\leq \aveOverInliers \normTwo{\vxx-\vxx\gt}^2 p^2( \normTwo{\MA_i\tran (\vxx-\vxx\gt)} )
 \leq \frac{\inlierRate^2 \eta^2}{4}
 \Big\}
\end{align}
concluding the proof.
\end{proof} % lemma

As a consequence, we can show that a constant fraction of $\vv_i \in \setInliers$ 
built by~\cref{algo:ldr} are close to $\vxx\gt$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Lemma 4.2 in~\cite{Karmalkar19neurips-ListDecodableRegression}] \label{lem:exists_vi}
For any $\pdist$ of degree $k$ satisfying $\axiomsLDR$, 
$\aveOverInliers \pExpect{\pdist}{\omega_i} \normTwo{\vv_i-\vxx\gt} \leq \frac{\inlierRate \eta}{2}$.
\end{lemma}
\begin{proof}% lemma
By~\cref{eq:boundxxgt}, we have $\axiomsLDR \sosimply{\vomega,\vxx}{t}
\left\{
\aveOverInliers \omega_i \normTwo{\vxx - \vxx\gt}^2 \leq \frac{\inlierRate^2 \eta^2}{4}
\right\}$.
We also have: $\axiomsLDR 
\sosimply{\vomega}{2} \{\omega_i^2 = \omega_i\}$ for any $i$. Therefore:\LC{also unclear}
\begin{align}
\axiomsLDR \sosimply{\vomega,\vxx}{k}
\left\{
\aveOverInliers \normTwo{ \omega_i\vxx -  \omega_i \vxx\gt}^2 \leq \frac{\inlierRate^2 \eta^2}{4}
\right\}
\end{align}
Since $\pdist$ satisfies $\axiomsLDR$, then it also satisfies:
\begin{align}
\aveOverInliers \pExpect{\pdist}{  
\normTwo{ \omega_i\vxx -  \omega_i \vxx\gt}^2} 
\leq \frac{\inlierRate^2 \eta^2}{4}
\end{align}
By \CS for pseudo-distributions, we get:\LC{how did the E pass inside?}
\begin{align}
\left( 
\aveOverInliers   
\normTwo{ \pExpect{\pdist}{ \omega_i\vxx } -  \pExpect{\pdist}{ \omega_i } \vxx\gt }
\right)^2
\leq 
\aveOverInliers 
\normTwo{ \pExpect{\pdist}{ \omega_i\vxx } -  \pExpect{\pdist}{ \omega_i } \vxx\gt }^2
 \leq \frac{\inlierRate^2 \eta^2}{4}
\end{align}
Since $\vv_i = \frac{\pExpect{\pdist}{\omega_i\vxx}}{\pExpect{\pdist}{\omega_i}}$ if $\pExpect{\pdist}{\omega_i} > 0$, or $\vv_i = \zero$ otherwise, we have
\begin{align}
\frac{1}{\setInliers} \sum_{i \in |\setInliers|, \pExpect{\pdist}{\omega_i} > 0} 
\pExpect{\pdist}{\omega_i} \normTwo{\vv_i - \vxx\gt}
 \leq \frac{\inlierRate \eta}{2}
\end{align}
concluding the proof.
\end{proof}% lemma

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Lemma 4.3 in~\cite{Karmalkar19neurips-ListDecodableRegression}]  \label{lem:sum_wi}
For any $\pdist$ of degree $\geq 4$ satisfying $\axiomsLDR$ that minimizes 
$\normTwo{\pExpect{\pdist}{\vomega}}$, $\sumOverInliers \pExpect{\pdist}{\omega_i} \geq \inlierRate^2 \nrMeasurements$.
\end{lemma}
\begin{proof}% lemma
Let $\vu = \frac{1}{\inlierRate \nrMeasurements} \pExpect{\pdist}{\vomega}$.
 Then, $\vu$ is a non-negative vector satisfying $\sumOverMeas u_i = 1$.
  Let $\wt(\setInliers) = \sumOverInliers u_i$ 
  and let $\wt(\setOutliers) = \sum_{i \notin \setInliers} u_i$. Then, 
  $\wt(\setInliers) + \wt(\setOutliers) = 1$. 
  By contradiction, we show that if $\wt(\setInliers) \leq \inlierRate$, then there exists 
  a pseudo-distribution $\pdist'$ satisfying $\axiomsLDR$ that achieves a lower value of 
  $\normTwo{\pExpect{\pdist}{\vomega}}$, hence contradicting optimality of $\pdist$. 

  Towards this goal, we define a third pseudo-distribution $\pdist\opt$ which is supported on a single $(\vomega,\vxx)$, the indicator $\ones_{\setInliers}$ and $\vxx\gt$. Therefore, $\pExpect{\pdist\opt}{\omega_i}=1$ iff $i\in\setInliers$ and zero otherwise. 
  Clearly, $\pdist\opt$ satisfies $\axiomsLDR$. Therefore, any convex combination $\pdist_\lambda = (1-\lambda) \pdist + \lambda \pdist\opt$ also satisfies $\axiomsLDR$. 
  We will show that whenever $\lambda >0$, then   $\normTwo{\pExpect{\pdist_\lambda}{\vomega}} < \normTwo{\pExpect{\pdist}{\vomega}}$.

  We first lower bound $\normTwo{\vxx}^2$ in terms of $\wt(\setInliers)$ and $\wt(\setOutliers)$.
  Observe that for any fixed values of  $\wt(\setInliers)$ and $\wt(\setOutliers)$, the minimum is attained by the vector
   $\vu$ that ensures $u_i =\frac{1}{\an} \wt(\setInliers)$ for each $i\in\setInliers$ and 
   $u_i =\frac{1}{(1-\inlierRate)\nrMeasurements} \wt(\setOutliers)$ otherwise. 

   This gives:
   \begin{align}
    \normTwo{\vu}^2 \geq 
    \left( \frac{\wt(\setInliers)}{\an} \right)^2 \an + 
    \left( \frac{1-\wt(\setInliers)}{(1-\inlierRate)\nrMeasurements} \right)^2 (1-\inlierRate)\nrMeasurements 
    \\ 
    = 
    \frac{1}{\an} \cdot \left( \wt(\setInliers)^2 + (1-\wt(\setInliers))^2 \left( \frac{\inlierRate}{1-\inlierRate} \right) \right)
    \end{align} 
	%
	Next, we compute the norm of $\vu' = \frac{1}{\an} \pExpect{\pdist_\lambda}{\vomega}$ as:
	\begin{align}
	\normTwo{\vu'}^2 = (1-\lambda)^2 \normTwo{\vu}^2 + 2\lambda(1-\lambda) \frac{\wt(\setInliers)}{\an} + \frac{\lambda^2}{\an} 
	\end{align}
	Thus:
	\begin{align}
	\normTwo{\vu'}^2 - \normTwo{\vu}^2 = (-2\lambda + \lambda^2) \normTwo{\vu}^2 
	+   \frac{\lambda^2}{\an} 
	+ 2\lambda(1-\lambda) \frac{\wt(\setInliers)}{\an}
	\\
	\leq 
	\frac{-2\lambda + \lambda^2}{\an} \left( 
	\wt(\setInliers)^2 + (1-\wt(\setInliers))^2 \frac{\inlierRate}{1-\inlierRate} 
 \right)
 + 2\lambda(1-\lambda) \frac{\wt(\setInliers)}{\an} + \frac{\lambda^2}{\an} 
	\end{align}
 	%
 	Rearranging:
 	\begin{align}
 	\normTwo{\vu}^2 - \normTwo{\vu'}^2 \geq \frac{\lambda}{\an} 
 	\left( 
 	(2-\lambda) 
 		\left( 
		\wt(\setInliers)^2 + (1-\wt(\setInliers))^2 \frac{\inlierRate}{1-\inlierRate} 
 		\right)
 	- \lambda - 2(1-\lambda) \wt(\setInliers)
 	\right)
 	\\
 	\geq
 	\frac{\lambda(2-\lambda)}{\an} 
 		\left( 
		\wt(\setInliers)^2 + (1-\wt(\setInliers))^2 \frac{\inlierRate}{1-\inlierRate}  - \wt(\setInliers)
 		\right)
 	\end{align}
 	%
 	Now whenever $\wt(\setInliers) < \inlierRate$, $\wt(\setInliers)^2 + (1-\wt(\setInliers))^2 \frac{\inlierRate}{1-\inlierRate}  - \wt(\setInliers) > 0$. Thus we can choose a small enough $\lambda > 0$ such that $\normTwo{\vu}^2 - \normTwo{\vu'}^2 > 0$.
\end{proof}% lemma

Using \cref{lem:exists_vi} and~\cref{lem:sum_wi} we can finally prove the correctness of~\cref{thm:highOut-apriori}.
First, since $\DistInliers$ is $k$-certifiably $(C,\frac{\an}{4C})$-anti-concentrated, Lemma 5.5 in~\cite{Karmalkar19neurips-ListDecodableRegression} implies that taking $\nrMeasurements \geq (k\dimAmbient)^{O(k)}$ 
samples ensures that $\setInliers$ is $k$-certifiably $(C,\frac{\an}{2C})$-anti-concentrated with 
probability at least $1-\frac{1}{\dimAmbient}$. Let's condition on this event in the following. 

Let $\pdist$ be a pseudo-distribution of degree $t$ satisfying $\axiomsLDR$ that minimizes 
$\normTwo{\pExpect{\pdist}{\vomega}}$. 
Such a pseudo-distribution exists since the set contains at least the distribution with $\omega_i = 1$ iff $i\in\setInliers$. 

From~\cref{lem:exists_vi}, we have $\aveOverInliers \pExpect{\pdist}{\omega_i} \normTwo{\vv_i - \vxx\gt} \leq 
\frac{\inlierRate \eta}{2}$. Let $Z = \frac{1}{\an} \aveOverInliers \pExpect{\pdist}{\omega_i}$. By a rescaling, we obtain:
\begin{align}
\frac{1}{\an} \aveOverInliers \frac{\pExpect{\dist}{\omega_i}}{Z} \normTwo{\vv_i - \vxx\gt} \leq 
\frac{1}{Z} \frac{\inlierRate \eta}{2}
\end{align}

Using~\cref{lem:sum_wi}, $Z \geq \inlierRate$. Therefore,
\begin{align}
\label{eq:proof31}
\frac{1}{\an} \aveOverInliers \frac{\pExpect{\dist}{\omega_i}}{Z} \normTwo{\vv_i - \vxx\gt} \leq 
\frac{\eta}{2}
\end{align}

Let $i \in [\nrMeasurements]$ be chosen with probability $\frac{\pExpect{\dist}{\omega_i}}{\an}$.
 Then, $\i \in\setInliers$ with probability $Z \geq \inlierRate$. 
 By Markov's inequality applied to~\eqref{eq:proof31}, with $\frac{1}{2}$ conditioned on $i \in\setInliers$, $\normTwo{\vv_i - \vxx\gt} \leq \eta$. Thus, in total, with probability at least $\frac{\inlierRate}{2}$, $\normTwo{\vv_i - \vxx\gt} \leq \eta$.
Thus, with probability at least $0.99$ over the draw of the random set $\List$, the list will contain an $\vxx$ 
such that $\normTwo{\vxx - \vxx\gt} \leq \eta$.
\end{proof} % theorem


==> lowOut-aPosteriori-TLS-noiseless.tex <==
\begin{theorem}[TLS Low-Outlier Case: A-Posteriori Estimation Contract with Noiseless Inliers]\label{thm:lowOut-aposterioriNoiselessTLS}
Assume the measurement set contains at least $\frac{\nrMeasurements + \minDim}{2}$ noiseless inliers, 
where $\minDim$ is the 
size of a minimal set. Moreover, assume that every subset of $\minDim$ inliers is \nondegenerate. 
% If the optimal solution of~\eqref{eq:MC} with $\barc = 0$ selects at least $0.5\nrMeasurements$ measurements as inliers (\ie has objective at least $0.5\nrMeasurements$), 
Then~\eqref{eq:TLS} with a sufficiently small $\barc > 0$ exactly recovers the unknown variable, $\vxx\tls = \vxx\gt$.  
\end{theorem}

\begin{proof}
Call 
$\measSet(\vxx\tls)$ the inlier set corresponding to an estimate 
$\vxx\tls$ (\ie $\measSet(\vxx\tls) \triangleq  \setdef{i\in[n]}{ \normTwo{\vy_i - \MA\tran \vxx\tls} \leq \barc }$). Moreover, define the TLS cost at $\vxx$ as:
\begin{align}
f(\vxx) = \sum_{ i \in \measSet(\vxx\tls) } \normTwo{ \vy_i - \MA_i \tran \vxx }^2 + \barcsq (\nrMeasurements- |\measSet(\vxx\tls)|)
\end{align} 
It is easy to see the TLS cost is the same as the objective in~\eqref{eq:TLS}.

We first prove that $|\measSet(\vxx\tls) | \geq \frac{\nrMeasurements + \minDim}{2}$. 
Towards this goal, we observe that $f(\vxx\gt) \leq \barcsq (\nrMeasurements- \frac{\nrMeasurements + \minDim}{2})$, which follows from the assumption that the inliers are noiseless and there are at least $\frac{\nrMeasurements + \minDim}{2}$ of them.
Now assume by contradiction that there exists an $\vxx\tls$ that solves~\eqref{eq:TLS} and is such that $|\measSet(\vxx\tls) | < \frac{\nrMeasurements + \minDim}{2}$. 
Such an estimate would achieve a cost:
\begin{align}
\label{eq:tlsCost}
f(\vxx\tls) = \sum_{ i \in \measSet(\vxx\tls) } \normTwo{ \vy_i - \MA_i \tran \vxx }^2 + \barcsq (\nrMeasurements- |\measSet(\vxx\tls)|) \\
 > \sum_{ i \in \measSet(\vxx\tls) } \normTwo{ \vy_i - \MA_i \tran \vxx }^2 + \barcsq 
 \left(\nrMeasurements- \frac{\nrMeasurements + \minDim}{2} \right) 
 \\
 \geq \barcsq \left(\nrMeasurements- \frac{\nrMeasurements + \minDim}{2} \right)
\end{align} 
which is larger than $f(\vxx\gt)$, hence contradicting optimality of $\vxx\tls$, and implying $|\measSet(\vxx\tls) | \geq \frac{\nrMeasurements + \minDim}{2}$.

Since both $|\measSet(\vxx\gt)|\geq \frac{\nrMeasurements + \minDim}{2}$ and $|\measSet(\vxx\tls)| \geq \frac{\nrMeasurements + \minDim}{2}$ then 
$|\measSet(\vxx\gt) \cap \measSet(\vxx\tls)| \geq \minDim$.
The subset of measurements $|\measSet(\vxx\gt) \cap \measSet(\vxx\tls)|$ are simultaneously solved by $\vxx\tls$ and $\vxx\gt$. 
Now if $\barc$ is selected to be small enough, $\sum_{ i \in \measSet(\vxx\tls) } \normTwo{ \vy_i - \MA_i \tran \vxx\tls }^2 = 0$. Therefore, $\vy_i = \MA_i \tran \vxx\tls$, $\forall i \in \measSet(\vxx\gt) \cap \measSet(\vxx\tls)$. At the same time, since the inliers are noiseless, $\vy_i = \MA_i \tran \vxx\gt$, $\forall i \in \measSet(\vxx\gt) \cap \measSet(\vxx\tls)$. 
Since every subset of $\minDim$ measurements is \nondegenerate, the two linear systems cannot have different solutions, hence $\vxx\tls = \vxx\gt$.
%it is not possible that there are two different estimates for that subset.
\end{proof}

==> lowOut-aPosterioriResults-backup.tex <==
%!TEX root = main.tex

\subsection{Naive Estimation Contracts with Low-Outlier Rates}
\label{sec:lowOut-aPosterioriResults}

\LC{mention that these are naive results: dimension-dependent: \url{https://arxiv.org/pdf/2002.05139.pdf}}

Before presenting the key results in this section, 
we need to remark that in all the estimation problems considered in this paper, we cannot reconstruct the 
unknown $\vxx$ from a single measurement, but we rather need a (sufficiently large) subset of measurements.

\begin{definition}[\Nondegenerate and Minimal Measurement Set]
A set $\measSet$ of measurements is \emph{\nondegenerate} if the following optimization problem admits a unique solution:
\begin{align}
\vxx_\measSet = \argmin_{\vxx \in \Domain} \sum_{i \in \measSet} \normTwo{ \vy_i - \MA_i\tran \vxx }^2
\end{align}
A \nondegenerate set of minimal size $\minDim$ is called a \emph{minimal} measurement set. 
\end{definition}

% In the noiseless case, 
Characterizations of the minimal sets for all the problems in Section~\ref{sec:motivatingProblems} are well known in the literature.
Indeed, a subfield of computer vision is specifically concerned with the design of \emph{minimal solvers}, which estimate the 
$\vxx$ from a minimal set of measurements.\footnote{The popularity of minimal solvers stems from their extensive use in outlier rejection schemes, such as RANSAC~\cite{Fischler81}.} 
For instance, the Wahba problem, the 3D registration problem, and the absolute problem 
require at least $\minDim = 3$ non-collinear points. 
On the other hand, the minimal set for multiple rotation averaging is a spanning tree of the rotation graph ($\minDim = N-1$).
%requires a subset of relative pose measurements that make the rotation graph connected.
% Note that the size 

The following theorem provides our first estimation contract, which establishes when~\eqref{eq:MC} recovers the true 
variable $\vxx\gt$ in the inliers are noiseless. 

\begin{theorem}[MC Low-Outlier Case: A-Posteriori Estimation Contract with Noiseless Inliers]\label{thm:lowOut-aposterioriNoiselessMC}
Assume the measurement set contains at least $\frac{\nrMeasurements + \minDim}{2}$ noiseless inliers, where $\minDim$ is the 
size of a minimal set. Moreover, assume that every subset of $\minDim$ inliers is \nondegenerate. 
% If the optimal solution of~\eqref{eq:MC} with $\barc = 0$ selects at least $0.5\nrMeasurements$ measurements as inliers (\ie has objective at least $0.5\nrMeasurements$), 
Then~\eqref{eq:MC} with $\barc = 0$ exactly recovers the unknown variable, $\vxx\maxCon = \vxx\gt$.  
\end{theorem}

\begin{proof}
Assume by contradiction that $\vxx\maxCon \neq \vxx\gt$ and call $\InlierSet$ and $\measSet\maxCon$ the true inliers and the set of inliers found by~\eqref{eq:MC} (\ie $\measSet\maxCon \doteq  \setdef{i\in[n]}{ \omega_i = 1 }$). 
Since $\InlierSet$ induces a feasible solution with cost $\frac{\nrMeasurements + \minDim}{2}$, by optimality 
it follows $|\measSet\maxCon| \geq \frac{\nrMeasurements + \minDim}{2}$.
Since $|\InlierSet|\geq \frac{\nrMeasurements + \minDim}{2}$ and $|\measSet\maxCon| \geq \frac{\nrMeasurements + \minDim}{2}$ then 
$|\InlierSet \cap \measSet\maxCon| \geq \minDim$.
Therefore, the subset of measurements $|\InlierSet \cap \measSet\maxCon|$ are simultaneously solved by $\vxx\maxCon$ and $\vxx\gt$. However, since every subset of $\minDim$ measurements is \nondegenerate, it is not possible that there are two different estimates for that subset.
\end{proof}

\cref{fig:maxConNoiseless} stresses the importance of \nondegeneracy in the estimation contract in \cref{thm:lowOut-aposterioriNoiselessMC}. The figure shows a simple linear regression problem in 3D where we need to fit a plane 
given 3D points belonging to the plane. In particular, we are given a set of $15$ measurements with $9$ inliers and $6$ outliers. While the set of inliers has size $\frac{\nrMeasurements + \minDim}{2} = 9$ (which satisfies one requirement in the theorem), there are subsets of degenerate points (in particular, the 4 collinear points at the intersection between the two planes). Intuitively, degenerate sets of measurements can be easily ``stolen'' by an adversary since they 
are compatible with multiple estimates of $\vxx$.

\begin{figure}[t!]
\centering
	\includegraphics[width=0.7\columnwidth, trim= 0mm 0mm 0mm 0mm, clip]{maxConNoiseless2} 
	\caption{Plane fitting with 9 inliers (green 3D points) and 6 outliers (red 3D points). 
	True plane is shown in black, while the plane computed by~\eqref{eq:MC} is shown in red. 
	When the estimation contract in~\cref{thm:lowOut-aposterioriNoiselessMC} is violated,~\eqref{eq:MC} 
	may fail to recover the variable $\vxx\gt$ even when given $\frac{\nrMeasurements + \minDim}
	{2}$ inliers.  \label{fig:maxConNoiseless}}
\end{figure}

The next theorem generalizes \cref{thm:lowOut-aposterioriNoiselessMC} to the case of noisy inliers.

\begin{theorem}[MC Low-Outlier Case: A-Posteriori Estimation Contract with Noisy Inliers]\label{thm:lowOut-aposterioriNoisyMC}
Assume the measurement set contains at least $\frac{\nrMeasurements + \minDim}{2}$ inliers, where $\minDim$ is the 
size of a minimal set. Moreover, assume that every subset of $\minDim$ inliers is \nondegenerate. 
Then~\eqref{eq:MC} produces an estimate $\vxx\maxCon$ such that 
$\normTwo{\vxx\maxCon - \vxx\gt} \leq \frac{2 \barc  \sqrt{\minDim \dimy}}{ \min_{ \calJ \subset \InlierSet, |\calJ|=\minDim } \sigma_\min(\MA_\calJ\tran) }$ where $\InlierSet$ is the set of inliers, $\MA_\calJ$ is the matrix obtained by stacking all submatrices $\MA_i$ for all $i \in \calJ$, and $\sigma_\min(\cdot)$ denotes the smallest singular value of a matrix.  
\end{theorem}

\begin{proof}
Let us call $\InlierSet$ and $\measSet\maxCon$ the true inliers and the set of inliers found by~\eqref{eq:MC} (\ie $\measSet\maxCon \doteq  \setdef{i\in[n]}{ \omega_i = 1 }$). 
Following beginning of the proof in~\cref{thm:lowOut-aposterioriNoiselessMC}, we conclude
 $|\InlierSet \cap \measSet\maxCon| \geq \minDim$; let us define $\calJ \doteq \InlierSet \cap \measSet\maxCon$. 
 Note that both $\vxx\gt$ and $\vxx\maxCon$ are feasible for~\eqref{eq:MC}, hence:
 \begin{align}
 \label{eq:boundsGT1}
 \max_{ i \in  \calJ} \normTwo{ \vy_i - \MA\tran_i \vxx\gt } \leq \barc \;\;\Longrightarrow \;\;
  \normInf{ \vy_\calJ - \MA\tran_\calJ \vxx\gt } \leq \barc 
  \\
   \label{eq:boundsMC1}
   \max_{ i \in  \calJ} \normTwo{ \vy_i - \MA\tran_i \vxx\maxCon } \leq \barc \;\;\Longrightarrow \;\;
  \normInf{ \vy_\calJ - \MA\tran_\calJ \vxx\maxCon } \leq \barc 
 \end{align} 
\LC{Using the triangle inequality and bounds~\eqref{eq:boundsGT1}-\eqref{eq:boundsMC1}: 
\begin{align}
\normInf{ (\vy_\calJ - \MA\tran_\calJ \vxx\gt) - (\vy_\calJ - \MA\tran_\calJ \vxx\maxCon) } \leq 
\normInf{ \vy_\calJ - \MA\tran_\calJ \vxx\gt } + \normInf{ \vy_\calJ - \MA\tran_\calJ \vxx\maxCon } \leq 2 \barc
\end{align}
Which after simplifying becomes:
\begin{align}
\normInf{  \MA\tran_\calJ (\vxx\maxCon - \vxx\gt) } \leq 2 \barc
\end{align}
}

\grayout{
 Now we want to use~\eqref{eq:boundsGT1} and~\eqref{eq:boundsMC1} to bound the distance between $\vxx\maxCon$ and $\vxx\gt$, and 
 let us call such a mismatch $\tilde{\vxx}$, \ie $\vxx\gt = \vxx\maxCon + \tilde{\vxx}$. Substituting this expression into~\eqref{eq:boundsMC1}:
 \begin{align}
 \label{eq:proof1}
 \normInf{ \vy_\calJ - \MA\tran_\calJ \vxx\gt + \MA\tran_\calJ \tilde{\vxx} } \leq \barc
 \end{align}
 Using the reverse triangle inequality:
  \begin{align}
\label{eq:proof2}
 \normInf{ \vy_\calJ - \MA\tran_\calJ \vxx\gt + \MA\tran_\calJ \tilde{\vxx} } \geq 
 \left| \normInf{ \MA\tran_\calJ \tilde{\vxx} } - \normInf{ \vy_\calJ - \MA\tran_\calJ \vxx\gt } \right|
 \end{align}
 Combining~\eqref{eq:proof1} and~\eqref{eq:proof2}:
\begin{align}
 \label{eq:proof3}
 & -\barc \leq \normInf{ \MA\tran_\calJ \tilde{\vxx} } - \normInf{ \vy_\calJ - \MA\tran_\calJ \vxx\gt } \leq \barc
 \\
 \text{(rearranging) }
 & -\barc + \normInf{ \vy_\calJ - \MA\tran_\calJ \vxx\gt } \leq \normInf{ \MA\tran_\calJ \tilde{\vxx} } \leq \barc +  \normInf{ \vy_\calJ - \MA\tran_\calJ \vxx\gt } \nonumber
 \\
 \text{(using~\eqref{eq:boundsGT1}) }
 & 0 \leq \normInf{ \MA\tran_\calJ \tilde{\vxx} } \leq 2 \barc  \nonumber
 \end{align}
 }
Using standard norm inequalities:
\begin{align}
 \label{eq:proof4}
\normInf{ \MA\tran_\calJ \tilde{\vxx} } \geq \frac{1}{\sqrt{\minDim \dimy}} \normTwo{ \MA\tran_\calJ \tilde{\vxx} }
\geq \frac{1}{\sqrt{\minDim }} \sigma_\min(\MA\tran_\calJ) \normTwo{\tilde{\vxx}}
\end{align}
Combining~\eqref{eq:proof4} and~\eqref{eq:proof3}:
 \begin{align}
 \label{eq:proof5}
\normTwo{\tilde{\vxx}} \leq \frac{  2 \barc \sqrt{\minDim \dimy}  }{  \sigma_\min(\MA\tran_\calJ)  }
\end{align}
Since we do not know which subset $\calJ$ was selected by~\eqref{eq:MC}, we take the  
set $\calJ$ of cardinality $\minDim$ attaining the smallest singular value across the set of inliers. 
Note that the assumption of \nondegeneracy implies that $\sigma_\min(\MA\tran_\calJ)$ remains nonzero.
\LC{is this true for manifold stuff?}
\end{proof}

\LC{these are naive bounds since they are dimension dependent}

We remark~\cref{thm:lowOut-aposterioriNoiselessMC} and~\cref{thm:lowOut-aposterioriNoisyMC} are ``a posterior'' contracts, 
since we cannot guarantee the computation of optimal solution is polynomial time, but we can apply them to certifiably optimal solutions.



\begin{theorem}[TLS Low-Outlier Case: A-Posteriori Estimation Contract with Noiseless Inliers]\label{thm:lowOut-aposterioriNoiselessTLS}
Assume the measurement set contains at least $\frac{\nrMeasurements + \minDim}{2}$ noiseless inliers, 
where $\minDim$ is the 
size of a minimal set. Moreover, assume that every subset of $\minDim$ inliers is \nondegenerate. 
% If the optimal solution of~\eqref{eq:MC} with $\barc = 0$ selects at least $0.5\nrMeasurements$ measurements as inliers (\ie has objective at least $0.5\nrMeasurements$), 
Then~\eqref{eq:TLS} with a sufficiently small $\barc > 0$ exactly recovers the unknown variable, $\vxx\tls = \vxx\gt$.  
\end{theorem}

\begin{proof}
Call 
$\measSet(\vxx\tls)$ the inlier set corresponding to an estimate 
$\vxx\tls$ (\ie $\measSet(\vxx\tls) \doteq  \setdef{i\in[n]}{ \normTwo{\vy_i - \MA\tran \vxx\tls} \leq \barc }$). Moreover, define the TLS cost at $\vxx$ as:
\begin{align}
f(\vxx) = \sum_{ i \in \measSet(\vxx\tls) } \normTwo{ \vy_i - \MA_i \tran \vxx }^2 + \barcsq (\nrMeasurements- |\measSet(\vxx\tls)|)
\end{align} 
It is easy to see the TLS cost is the same as the objective in~\eqref{eq:TLS}.

We first prove that $|\measSet(\vxx\tls) | \geq \frac{\nrMeasurements + \minDim}{2}$. 
Towards this goal, we observe that $f(\vxx\gt) \leq \barcsq (\nrMeasurements- \frac{\nrMeasurements + \minDim}{2})$, which follows from the assumption that the inliers are noiseless and there are at least $\frac{\nrMeasurements + \minDim}{2}$ of them.
Now assume by contradiction that there exists an $\vxx\tls$ that solves~\eqref{eq:TLS} and is such that $|\measSet(\vxx\tls) | < \frac{\nrMeasurements + \minDim}{2}$. 
Such an estimate would achieve a cost:
\begin{align}
\label{eq:tlsCost}
f(\vxx\tls) = \sum_{ i \in \measSet(\vxx\tls) } \normTwo{ \vy_i - \MA_i \tran \vxx }^2 + \barcsq (\nrMeasurements- |\measSet(\vxx\tls)|) \\
 > \sum_{ i \in \measSet(\vxx\tls) } \normTwo{ \vy_i - \MA_i \tran \vxx }^2 + \barcsq 
 \left(\nrMeasurements- \frac{\nrMeasurements + \minDim}{2} \right) 
 \\
 \geq \barcsq \left(\nrMeasurements- \frac{\nrMeasurements + \minDim}{2} \right)
\end{align} 
which is larger than $f(\vxx\gt)$, hence contradicting optimality of $\vxx\tls$, and implying $|\measSet(\vxx\tls) | \geq \frac{\nrMeasurements + \minDim}{2}$.

Since both $|\measSet(\vxx\gt)|\geq \frac{\nrMeasurements + \minDim}{2}$ and $|\measSet(\vxx\tls)| \geq \frac{\nrMeasurements + \minDim}{2}$ then 
$|\measSet(\vxx\gt) \cap \measSet(\vxx\tls)| \geq \minDim$.
The subset of measurements $|\measSet(\vxx\gt) \cap \measSet(\vxx\tls)|$ are simultaneously solved by $\vxx\tls$ and $\vxx\gt$. 
Now if $\barc$ is selected to be small enough, $\sum_{ i \in \measSet(\vxx\tls) } \normTwo{ \vy_i - \MA_i \tran \vxx\tls }^2 = 0$. Therefore, $\vy_i = \MA_i \tran \vxx\tls$, $\forall i \in \measSet(\vxx\gt) \cap \measSet(\vxx\tls)$. At the same time, since the inliers are noiseless, $\vy_i = \MA_i \tran \vxx\gt$, $\forall i \in \measSet(\vxx\gt) \cap \measSet(\vxx\tls)$. 
Since every subset of $\minDim$ measurements is \nondegenerate, the two linear systems cannot have different solutions, hence $\vxx\tls = \vxx\gt$.
%it is not possible that there are two different estimates for that subset.
\end{proof}

\begin{theorem}[TLS Low-Outlier Case: A-Posteriori Estimation Contract with Noisy Inliers]\label{thm:lowOut-aposterioriNoisyTLS}
Assume the squared residual error for the inliers is $\gamma$, \ie $\sum_{ i \in \InlierSet } \normTwo{ \vy_i - \MA_i \tran \vxx\gt }^2 = \gamma$, where $\InlierSet$ is the set of inliers.
Moreover, assume the measurement set contains at least $\frac{\nrMeasurements + \minDim}{2} + \frac{\gamma}{\barcsq}$ 
inliers, where $\minDim$ is the 
size of a minimal set, and that every subset of $\minDim$ inliers is \nondegenerate. 
Then~\eqref{eq:TLS} produces an estimate $\vxx\tls$ such that 
$\normTwo{\vxx\tls - \vxx\gt} \leq \frac{2 \barc  \sqrt{\minDim \dimy}}{ \min_{ \calJ \subset \InlierSet, |\calJ|=\minDim } \sigma_\min(\MA_\calJ\tran) }$ where $\MA_\calJ$ is the matrix obtained by stacking all submatrices $\MA_i$ for all $i \in \calJ$, and $\sigma_\min(\cdot)$ denotes the smallest singular value of a matrix.  
\end{theorem}

\begin{proof}
Call 
$\measSet(\vxx\tls)$ the inlier set corresponding to an estimate 
$\vxx\tls$ (\ie $\measSet(\vxx\tls) \doteq  \setdef{i\in[n]}{ \normTwo{\vy_i - \MA\tran \vxx\tls} \leq \barc }$). Moreover, define the TLS cost at $\vxx$ as in~\eqref{eq:tlsCost}.

We first prove that $|\measSet(\vxx\tls) | \geq \frac{\nrMeasurements + \minDim}{2}$. 
Towards this goal, we observe that $f(\vxx\gt) \leq \gamma + \barcsq (\nrMeasurements- \frac{\nrMeasurements + \minDim}{2} - \frac{\gamma}{\barcsq}) = \barcsq (\nrMeasurements- \frac{\nrMeasurements + \minDim}{2})$, which follows from the assumption that the inliers have squared residual error $\gamma$  and there are at least $\frac{\nrMeasurements + \minDim}{2} + \frac{\gamma}{\barcsq}$ of them.
Now assume by contradiction that there exists an $\vxx\tls$ that solves~\eqref{eq:TLS} and is such that $|\measSet(\vxx\tls) | < \frac{\nrMeasurements + \minDim}{2}$. 
Such an estimate would achieve a cost:
\begin{align}
f(\vxx\tls) = \sum_{ i \in \measSet(\vxx\tls) } \normTwo{ \vy_i - \MA_i \tran \vxx }^2 + \barcsq (\nrMeasurements- |\measSet(\vxx\tls)|) \\
 > \sum_{ i \in \measSet(\vxx\tls) } \normTwo{ \vy_i - \MA_i \tran \vxx }^2 + \barcsq 
 \left(\nrMeasurements- \frac{\nrMeasurements + \minDim}{2} \right) 
 \\
 \geq \barcsq \left(\nrMeasurements- \frac{\nrMeasurements + \minDim}{2} \right)
\end{align} 
which is larger than $f(\vxx\gt)$, hence contradicting optimality of $\vxx\tls$, and implying $|\measSet(\vxx\tls) | \geq \frac{\nrMeasurements + \minDim}{2}$.

Since both $|\measSet(\vxx\gt)|\geq \frac{\nrMeasurements + \minDim}{2}$ and $|\measSet(\vxx\tls)| \geq \frac{\nrMeasurements + \minDim}{2}$ then 
$|\measSet(\vxx\gt) \cap \measSet(\vxx\tls)| \geq \minDim$.
The subset of measurements $|\measSet(\vxx\gt) \cap \measSet(\vxx\tls)|$ are simultaneously solved by $\vxx\tls$ and $\vxx\gt$. 
Then following the same line of thoughts as in the proof of~\cref{thm:lowOut-aposterioriNoisyMC}, we prove the claim.
% Now if $\barc$ is selected to be small enough, $\sum_{ i \in \measSet(\vxx\tls) } \normTwo{ \vy_i - \MA_i \tran \vxx\tls }^2 = 0$. Therefore, $\vy_i = \MA_i \tran \vxx\tls$, $\forall i \in \measSet(\vxx\gt) \cap \measSet(\vxx\tls)$. At the same time, since the inliers are noiseless, $\vy_i = \MA_i \tran \vxx\gt$, $\forall i \in \measSet(\vxx\gt) \cap \measSet(\vxx\tls)$. 
% Since every subset of $\minDim$ measurements is \nondegenerate, the two linear systems cannot have different solutions, hence $\vxx\tls = \vxx\gt$.
%it is not possible that there are two different estimates for that subset.
\end{proof}

==> lowOut-aPrioriResults-LTS-closerToKlivan.tex <==
%!TEX root = main.tex

\subsubsection{Contracts for~\eqref{eq:LTS}}
\label{sec:lowOut-aPrioriResults-LTS}

results from Klivans, extended to vector-valued measurements.

Let
$\DistInliers$: true inlier distribution.
$\DistSampleInliers$: uniform distribution over sampled inliers.

\begin{align}
\label{eq:errorAtx}
\err_\DistInliers(\vxx) = \Expect{ \DistInliers }{ \residual{\vxx}^2  }
\end{align}

\begin{align}
\label{eq:sampleErrorAtx}
\err_\DistSampleInliers(\vxx) = \aveOverMeas \residuali{\vxx}^2 
\end{align}

\begin{align}
\label{eq:errorAtx}
\trimmederr_\DistInliers(\vxx) = \Expect{ \DistInliers }{ \normTwo{\vy - \trim_M(\MA\tran \vxx) }^2  }
\end{align}
where $\trim_M$ clips the entries of a vector between $[-M,M]$.

\begin{align}
\label{eq:optx}
\optt_\DistInliers = \min_{\vxx \in \Domain} \err_\DistInliers(\vxx), \qquad 
\vxx\gt = \argmin_{\vxx \in \Domain} \err_\DistInliers(\vxx)
\end{align}

For a real random variable $a \in \Real{}$, $\normk{a} = \Expect{}{a^k}^{\frac{1}{k}}$.

\begin{definition}[Certifiable Hypercontractivity]
to be adjusted to vector-valued setup. Maybe with inner product and $\normFrob{\MV} = 1$?
\LC{to be added}
\end{definition}

many distributions are c.h.


\begin{align}
\label{eq:LTS2}
\vxx_\lts = \argmin_{ \substack{ \vomega \in \{0;1\}^\nrMeasurements \\ \vxx \in \Domain } } 
& \left(\aveOverMeas \omega_i \normTwo{ \vy_i - \MA_i \tran \vxx }^2 \right)^2 \\
\subject & \sumOverMeas{\omega_i} = \alpha \nrMeasurements \nonumber
\end{align}

\begin{align}
\label{eq:LTS-SDP-k}
\tag{LTS-SDP-k}
\text{define relaxation}
\Longrightarrow
\vxx\ltssdp = \MM_{\vxx} 
\\
\text{optimal cost defined: } \opttsos^2
\end{align}

\begin{theorem}[Low-Outlier Case: Estimation Contract, adapted from  Theorem 5.1 in~\cite{Klivans18arxiv-robustRegression}]
\label{thm:lowOut-apriori-LTS}
Let $\DistInliers$ be the (inlier) distribution on $\Real{\dimAmbient} \times [-M,M]^\dimy$ for some positive $M \in \Real{}$, such that the marginal on $\Real{\dimAmbient}$ is a $(C,4)$-certifiably hypercontractive distribution. 
Let $\optt_{\DistInliers,B} = \min_{\vxx \in \Domain} \Expect{ \DistInliers }{ \residual{\vxx}^2  }$ 
where the minimum is over all $\vxx$ of bit complexity $B$, and let $\vxx\opt$ be any such minimizer.
For some outlier rate $\outlierRate$ and $\epsilon > 0$, consider a $\outlierRate$-corrupted sample with 
$\nrMeasurements \geq \text{poly}(\dimAmbient^4, B, M, \frac{1}{\epsilon})$ measurements, where the inliers are drawn from $\DistInliers$.
Then, with probability at least $1-\epsilon$ (over the drawing of the samples), the convex relaxation~\eqref{eq:LTS-SDP-k} with $k=4$ outputs $\vxx\ltssdp$ such that for $\kappa = C(2)$:
\begin{align}
\trimmederr_\DistInliers( \vxx\ltssdp ) < 
(1 + O(\kappa) \sqrt{\outlierRate}  ) \optt_{\DistInliers,B}
+
O(\kappa) \sqrt{\outlierRate}  \sqrt{ \Expect{\DistInliers}{  \residual{\vxx\gt}^4 } } + \epsilon
\end{align}
\end{theorem}

Comment: 
- bound is about stating that the error of the relaxation is not much larger than the error of the best estimate given inliers 
$\optt_{\DistInliers,B}$ plus some higher order moments
- level 4 is impractical
- bounds M and bounded bit complexity is mostly to derive generalization bounds

%=================================================================
\subsubsection{Bounding the Optimization Error}

We first bound the empirical error over the given samples $\DistSampleInliers$ (this essentially is a statement
about the tightness of the relaxation):

\begin{lemma}[Bounding the optimization error, adapted from Lemma 5.3 in~\cite{Klivans18arxiv-robustRegression}]
\label{lem:boundingOptError}
Under the assumptions of~\cref{thm:lowOut-apriori-LTS}, with probability at least $1-\epsilon$, 
\begin{align}
\err_{\DistSampleInliers}(\vxx\ltssdp) \leq 
(1 + O(\kappa)\sqrt{\outlierRate}  ) \optt\ltssdp
+
O(\kappa) \sqrt{\outlierRate}  \sqrt{ \Expect{\DistSampleInliers}{  \residuali{\vxx\gt}^4 } } 
\end{align}
\end{lemma}

\begin{proof}
 \myParagraph{\sos Proof of Robust Certifiability (Lemma 5.6 in~\cite{Klivans18arxiv-robustRegression})}
 We now show that any set of variables that are feasible for~\eqref{eq:LTS}, also satisfy 
 an error bound. Here we use an \sos proof system, that allows performing logical deductions from polynomial constraints. In particular, let us define the constraint set in problem~\eqref{eq:LTS}:
\begin{align}
\calA \doteq \left\{
\begin{array}{cl}
\omega_i^2 = \omega_i, \;\; i=1,\ldots,\nrMeasurements \\ 
\vxx \in \Domain \\
\sumOverMeas{\omega_i} = \alpha \nrMeasurements 
\end{array}
\right\}
\end{align}
where we noted that the constraint $\vomega_i \in \{0;1\}$ is the same as imposing $\omega_i^2 = \omega_i$.
Defining 
\begin{align}
\label{eq:err_w_x}
\err(\vomega,\vxx) \doteq \aveOverMeas \omega_i \residuali{\vxx}^2,
\end{align}
 now we prove that the error of any solution that satisfies $\calA$ cannot be very far from the empirical error for the inliers:
 \begin{align}
 \label{eq:sosRobustCertifiability}
\calA \sosimply{\vxx}{k}
( \err_{\DistSampleInliers(\vxx)} - \err(\vomega,\vxx) )^2
\leq 
\outlierRate 2^{\Theta(4)} \kappa^4 \err(\vomega,\vxx)^2 +
\outlierRate 2^{\Theta(4)} \kappa^4 \left(\frac{1}{\nrMeasurements} \sumOverMeas 
\normTwo{\vy_i - \MA_i\tran \vxx\opt}^4 \right)  
% (1 + a \kappa \outlierRate^{1 - \frac{2}{k}}  ) \optt\ltssdp
% +
%  a \kappa \outlierRate^{1 - \frac{2}{k}}  \sqrt{ \Expect{\DistSampleInliers}{  \residual{\vxx\gt}^4 } } 
\end{align}
with the bit complexity of the proof being polynomial in $\nrMeasurements$ and $\dimAmbient^4$.
The proof is involved, but it is the crux of the result.

For a given $\vomega$ that satisfies $\calA$, let $\vomega'$ be such that $\omega_i' = \omega_i$ iff 
$i$ is an inlier and $\omega_i = 0$ otherwise (intuitively, $\vomega'$ is the indicator for subset of the selected measurements $\vomega$ that are inliers). %$\omega_i = 1$ are the inliers
Define $\vy_i' = \vy_i$ and $\MA_i' = \MA_i$ if $\omega_i' = 1$ or set $\vy_i' = \zero$ and $\MA_i' = \zero$ otherwise.
Note that $\sumOverMeas \omega_i' \geq (1-2\outlierRate) \nrMeasurements$ (the two sets, each of size $(1-2\outlierRate)$ cannot deviate from more than $2\outlierRate$). 
Then
\begin{align}
\label{eq:overlapBound}
\explanation{ \aveOverMeas (1-\omega_i')^2 \overbrace{=}^{\text{binary var.}} \aveOverMeas (1-\omega_i') = 1 - \aveOverMeas \omega_i' \leq 1 - (1-2 \beta) }
\sosimply{\vomega'}{2} \left\{ \aveOverMeas (1-\omega_i')^2 \leq 2\outlierRate \right\}
\end{align}
We have:
\begin{align}
\sosimply{ \red{\vomega},\vxx}{4} \left\{ 
\err_{\DistSampleInliers}(\vxx) = 
\overbrace{
\aveOverMeas \omega_i' \residuali{\vxx}^2
}^{\text{error for selected inliers}} +
\overbrace{
\aveOverMeas (1-\omega_i') \residuali{\vxx}^2
}^{\text{error for all other measurements }}
 \right\}
\end{align}

On the other hand, we also have (since other measurements with $\omega_i'=0$ can only add positive terms): 
\begin{align}
\sosimply{ \red{\vomega},\vxx}{4} 
\aveOverMeas \omega_i' \residuali{\vxx}^2 \leq
\aveOverMeas \normTwo{ \vy_i' - (\MA_i')\tran \vxx }^2 = \err_{\DistInliers'}(\vxx)
\end{align}
Combining the above and using the \sos version of \HoldersInequality:
% (in the first equality 
% below we note that for $\omega_i=1, (\vy_i' ,\MA_i')$ match $(\vy_i,\MA_i)$ or those are zero otherwise):
\begin{align}
\sosimply{ \red{\vomega},\vxx}{4} 
(\err_\DistSampleInliers(\vxx) - \err_{\DistInliers'}(\vxx) )^2
= 
\overbrace{\left(
\aveOverMeas (1-\omega_i') \residuali{\vxx}^2
\right)^2}^{ \text{cost of outliers selected by $\vomega'$} }
\\
\leq 
\overbrace{
\left( \aveOverMeas (1-\omega_i') \right) 
\left( \aveOverMeas \residual{\vxx}^4 \right)
}^{\text{using~\eqref{eq:holder2_1}}}
\\
\leq 
\overbrace{
2\outlierRate
}^{\text{using~\eqref{eq:overlapBound}}}
\left( \aveOverMeas \residuali{\vxx}^4 \right) \label{eq:proof13}
\end{align}

Now we notice that:
\begin{align}
\left( \aveOverMeas \residuali{\vxx}^4 \right) = 
\left( \aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx + \MA_i\tran \vxx\gt - \MA_i\tran \vxx\gt }^4 \right) =
\\
=  \aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx\gt - \MA_i\tran (\vxx - \vxx\gt)  }^4 
\leq \quad\text{(via \red{\sos?} triangle inequality)} \\
 \aveOverMeas \left( \normTwo{ \vy_i - \MA_i\tran \vxx\gt } + \normTwo{\MA_i\tran (\vxx - \vxx\gt)} \right)^4
\end{align}

Next, using the \sos inequality $(a+b)^4 \leq 2^4 a^4 + 2^4 b^4$ summand-wise:
\begin{align}
\sosimply{ \vxx }{4}
\left( \aveOverMeas \residuali{\vxx}^4 \right) 
\leq 
\aveOverMeas \left( \normTwo{ \vy_i - \MA_i\tran \vxx\gt } + \normTwo{\MA_i\tran (\vxx - \vxx\gt)} \right)^4
\\
\leq
2^4  \aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx\gt }^4
+
2^4 \aveOverMeas \normTwo{ \MA_i\tran (\vxx - \vxx\gt)}^4 \label{eq:proof11}
\end{align}
By certifiable hypercontractivity of $\DistSampleInliers$:
\begin{align}
\sosimply{ \vxx }{4} \aveOverMeas \normTwo{ \MA_i\tran (\vxx - \vxx\gt)}^4 
 \leq C(2)^2 \left( \aveOverMeas \normTwo{ \MA_i\tran (\vxx - \vxx\gt)}^2 \right)^2 
\end{align}
Now we notice that:
\begin{align}
\left( \aveOverMeas \normTwo{ \MA_i\tran (\vxx - \vxx\gt)}^2 \right)^2 =
\left( \aveOverMeas \normTwo{ -\vy_i + \MA_i\tran \vxx + \vy_i - \MA_i\tran \vxx\gt }^2 \right)^2 
\\
\leq \quad\text{(via \red{\sos?} triangle inequality)} 
\\  
\left( \aveOverMeas (\normTwo{ \vy_i - \MA_i\tran \vxx} + \normTwo{\vy_i - \MA_i\tran \vxx\gt })^2 \right)^2 
\end{align}

By using again the \sos inequality $(a+b)^2 \leq 2^2 a^2 + 2^2 b^2$ summand-wise:
\begin{align}
\sosimply{ \vxx }{4}
\left( \aveOverMeas (\normTwo{ \vy_i - \MA_i\tran \vxx} + \normTwo{\vy_i - \MA_i\tran \vxx\gt })^2 \right)^2 
\\
\leq 2^2 \left( \aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx}^2 \right)^2
+
2^2 \left( \aveOverMeas \normTwo{\vy_i - \MA_i\tran \vxx\gt }^2 \right)^2 \label{eq:proof12}
\end{align}

Finally, using again the \sos version of \HoldersInequality
\begin{align}
\sosimply{ \vxx }{4}
\left( \aveOverMeas \normTwo{\vy_i - \MA_i\tran \vxx\gt }^2 \right)^2 
\leq 
\overbrace{ 
 \aveOverMeas \normTwo{\vy_i - \MA_i\tran \vxx\gt }^4 
 }^{\text{using \red{$f=\normTwo{\vy_i - \MA_i\tran \vxx\gt}^2$ and $g=1$ and $p=2$ and $q=1$}}}
\end{align}

Combining the above with~\eqref{eq:proof11}: 
\begin{align}
\sosimply{ \vxx }{4}
\left( \aveOverMeas \residual{\vxx}^4 \right) 
\leq 
2^4  \aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx\gt }^4
\\
+
2^4 C(2)^2 
\left(
 2^2 \left( \aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx}^2 \right)^2
+
2^2 \aveOverMeas \normTwo{\vy_i - \MA_i\tran \vxx\gt }^4 
\right)
\\
=
(2^4+ 2^6 C(2)^2 ) \left( \aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx\gt }^4 \right)
+
2^6 C(2)^2 \left( \overbrace{\aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx}^2}^{\err_\DistSampleInliers(\vxx)} \right)^2
\end{align}
Hence, together with~\eqref{eq:proof13}:
\begin{align}
\sosimply{ \red{\vomega},\vxx}{4} 
(\err_\DistSampleInliers(\vxx) - \err_{\DistInliers'}(\vxx) )^2
\leq 
(2\outlierRate) 2^6 C(2)^2 \left( \err_\DistSampleInliers(\vxx) \right)^2
\\
+
(2\outlierRate) (2^4+ 2^6 C(2)^2 ) \left( \aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx\gt }^4 \right)
\end{align}

Using the \sos inequality $a^k \leq 2^k (a-b)^k + 2 b^k$ (which holds for any $a,b$ and any even $k$) and applying it with $a = \err_\DistSampleInliers(\vxx)$, 
$b = \err_{\DistInliers'}(\vxx)$, and rearranging the terms: % and $\delta = (2\outlierRate)^2 2^6 C(4)^2$:
\begin{align}
\sosimply{ \red{\vomega},\vxx}{4} 
(1 - (2\outlierRate) 2^8 C(2)^2 )
(\err_\DistSampleInliers(\vxx) - \err_{\DistInliers'}(\vxx) )^2
\\
\leq 
(2\outlierRate) 2^8 C(2)^2 \left( \err_{\DistInliers'}(\vxx) \right)^2
\\
+
(2\outlierRate) (2^4+ 2^6 C(2)^2 ) \left( \aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx\gt }^4 \right)
\end{align}
%
which finally implies
\begin{align}
\sosimply{ \red{\vomega},\vxx}{4} 
(\err_\DistSampleInliers(\vxx) - \err_{\DistInliers'}(\vxx) )^2
\\
\leq 
\frac{(2\outlierRate) 2^8 C(2)^2}{(1 - (2\outlierRate) 2^8 C(2)^2 )} 
\left( \err_{\DistInliers'}(\vxx) \right)^2
\\
+
\frac{(2\outlierRate) (2^4+ 2^6 C(2)^2 )}{(1 - (2\outlierRate) 2^8 C(2)^2 )} \left( \aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx\gt }^4 \right)
\end{align}



% \myParagraph{Hypercontractivity of uniform distribution over sample set}
Finally, we recall (Lemma 5.7 in~\cite{Klivans18arxiv-robustRegression}) that if $\DistInliers$ 
is a $(C,k)$-certifiably hypercontractive distribution on $\Real{\dimAmbient}$ 
 and we draw at least $\nrMeasurements \geq \Omega( (\dimAmbient^{\frac{k}{2}} \log(\dimAmbient/\delta))^{\frac{k}{2}} )$, then the uniform distribution over the sample $\DistSampleInliers$ is 
 $(2C,k)$-certifiably hypercontractive.

 \myParagraph{Completing the proof}
Consider a pseudo-distribution $\pdist$ that satisfies $\calA$. 
Using the \sos proof in~\eqref{eq:sosRobustCertifiability} we conclude:
 \begin{align}
\pExpect{\pdist}{ ( \err_{\DistSampleInliers(\vxx)} - \err(\vomega,\vxx) )^2}
\leq 
\outlierRate 2^{\Theta(4)} \kappa^4 
\overbrace{ \pExpect{\pdist}{\err(\vomega,\vxx)^2} }^{\text{by definition: }\opttsos^2}+
\outlierRate 2^{\Theta(4)} \kappa^4
\overbrace{ \left(\frac{1}{\nrMeasurements} \sumOverMeas 
\normTwo{\vy_i - \MA_i\tran \vxx\opt}^4 \right) }^{\text{by definition: }\widehat{\optt_4}^2}  
\end{align}
Taking the square root of both sides and recalling that $\sqrt{a+b} \leq \sqrt{a} + \sqrt{b}$:
% https://math.stackexchange.com/questions/318649/square-root-of-a-sum-bound 
 \begin{align}
\sqrt{  \pExpect{\pdist}{ ( \err_{\DistSampleInliers(\vxx)} - \err(\vomega,\vxx) )^2} }
\leq 
\sqrt{ \outlierRate 2^{\Theta(4)} \kappa^4 }
\opttsos+
\sqrt{  \outlierRate 2^{\Theta(4)} \kappa^4  } 
\widehat{\optt_4}
\end{align}
Now using the \sos version of \HoldersInequality we get 
$\pExpect{\pdist}{ \err_{\DistSampleInliers(\vxx)} - \err(\vomega,\vxx)}^2 \leq
\pExpect{\pdist}{ ( \err_{\DistSampleInliers(\vxx)} - \err(\vomega,\vxx) )^2}$:
\begin{align}
\pExpect{\pdist}{ ( \err_{\DistSampleInliers(\vxx)} - \err(\vomega,\vxx) ) }
\leq 
\sqrt{ \outlierRate 2^{\Theta(4)} \kappa^4 }
\opttsos+
\sqrt{ \outlierRate 2^{\Theta(4)} \kappa^4 } 
\widehat{\optt_4}
\\
\pExpect{\pdist}{ \err_{\DistSampleInliers(\vxx)} }
\leq
\overbrace{ 
\pExpect{\pdist}{ \err(\vomega,\vxx) }
}^{\red{\text{unclear why this disappears as} \opttsos}}
+
\sqrt{ \outlierRate 2^{\Theta(4)} \kappa^4 }
\opttsos+
\sqrt{ \outlierRate 2^{\Theta(4)} \kappa^4} 
\widehat{\optt_4}  
\end{align}
Hence:
\begin{align}
\pExpect{\pdist}{ \err_{\DistSampleInliers(\vxx)} }
\leq
(1 + \sqrt{ \outlierRate 2^{\Theta(4)} \kappa^4  } )
\opttsos+
\sqrt{ \outlierRate 2^{\Theta(4)} \kappa^4 } 
 \widehat{\optt_4}  
\end{align}
Applying \sos \HoldersInequality one last time $  \err_{\DistSampleInliers} (\pExpect{\pdist}{ \vxx} )  \leq \pExpect{\pdist}{ \err_{\DistSampleInliers(\vxx)} } $ leading to:
\begin{align}
\err_{\DistSampleInliers} (\pExpect{\pdist}{ \vxx} )
\leq
(1 + \sqrt{ \outlierRate 2^{\Theta(4)} \kappa^4 } )
\opttsos+
\sqrt{ \outlierRate 2^{\Theta(4)} \kappa^4 } 
\widehat{\optt_4} 
\end{align}
which proves the claim.

\end{proof}

%=================================================================
\subsubsection{Bounding the Generalization Error}

\begin{lemma}[Bounding the generalization error, adapted from Lemma 5.4 in~\cite{Klivans18arxiv-robustRegression}]
\label{lem:boundingGenError}
Under the assumptions of~\cref{thm:lowOut-apriori-LTS}, with probability at least $1-\epsilon$, the following hold: 
\begin{align}
 \optt\ltssdp &\leq \optt_\DistInliers + \epsilon \label{eq:proof-claim1} \\
 \trimmederr_\DistInliers( \vxx\ltssdp ) &\leq \err_{\DistSampleInliers}(\vxx\ltssdp) + \epsilon \label{eq:proof-claim2} 
\end{align}
\end{lemma}

\begin{proof}
We start by observing that:
\begin{align}
\label{eq:proof-bound1}
\opttsos^2 \leq \err_{\DistSampleInliers}(\vxx^\gt)^2, 
\end{align}
which follows from the fact that the 
SDP is a relaxation ($\opttsos^2$ is the optimal objective of the relaxations).

Now we argue that $\err_{\DistSampleInliers}(\vxx^\gt)$ must be sufficiently close to $\err_{\DistInliers}(\vxx^\gt)$
 assuming the sample size is large enough. 
 Let us define a random variable $Z \doteq \normTwo{ \vy - \MA\tran \vxx\gt }^2$.
 Let us first bound the variance of $Z$:
 \begin{align}
 \explanation{ \|x+y\|^4 = (\|x+y\|^2)^2 \overbrace{\leq}^{triangle ineq.}  (\|x\|^2+ \|y\|^2)^2 \overbrace{\leq}^{triangle ineq.}  \|x\|^4+ \|y\|^4   }
 \Expect{}{ Z^2 } = 
 \Expect{}{  \normTwo{ \vy - \MA\tran \vxx\gt }^4 } 
  \leq  \Expect{}{  \normTwo{ \vy}^4 } + \Expect{}{  \normTwo{ \MA\tran \vxx\gt }^4 } 
  \leq 2M^4 + 2 C^2  \Expect{}{  \normTwo{ \MA\tran \vxx\gt }^2 }^2 
 \end{align}
 where in the last inequality we used hypercontractivity. 
 Now:
  \begin{align} 
 \red{ 
  \Expect{}{  \normTwo{ \MA\tran \vxx\gt }^2 } \leq  2 
   \Expect{}{  \normTwo{ \vy - \MA\tran \vxx\gt }^2 } + 2 
    \Expect{}{  \normTwo{ \vy }^2 } 
    } 
 \leq 
 2 \optt_{\DistInliers} + 2M^2 \leq 4M^2
\end{align}
where we used $\optt_{\DistInliers} \leq M^2$ (since the zero function achieves this error?).
Thus if we take at least $O(1/\epsilon^3)\cdot M^4$ samples, then (\LC{to check why})
\begin{align}
\prob{ 
\left| 
\aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx\gt }^2 - \Expect{}{\normTwo{ \vy - \MA\tran \vxx\gt }^2}   
\right| \geq \epsilon} \leq \epsilon
\end{align}
thus with probability at least $1-\epsilon$, we have
 \begin{align}
 \left| 
\aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx\gt }^2 - \Expect{}{\normTwo{ \vy - \MA\tran \vxx\gt }^2}  
\right| \leq \epsilon \\ 
\overbrace{\aveOverMeas \normTwo{ \vy_i - \MA_i\tran \vxx\gt }^2 }^{\err_{\DistSampleInliers}(\vxx\gt) } 
\leq 
\overbrace{ \Expect{}{\normTwo{ \vy_i - \MA_i\tran \vxx\gt }^2} }^{\optt_{\DistInliers} }  +  \epsilon
\label{eq:proof-bound2}
\end{align}
combining~\eqref{eq:proof-bound1} and \eqref{eq:proof-bound2} proves the first part of the claim~\eqref{eq:proof-claim1}.

In order to prove the second and last part of the claim, \ie eq.~\eqref{eq:proof-claim2}, 
we can use standard generalization arguments, such as the following claim:

\begin{fact}[Consequence of Theorem 10.1 in \red{[MRT12]}] 
Let H we a class of functions over $\Real{\dimAmbient}$ such that each $h \in H$ can be described in B bits.
Suppose each function in H takes values in $[-M,+M]$ for some positive $M$. 
Let $\DistInliers$ be a distribution on $\Real{\dimAmbient} \times [-M,+M]$ and consider $\nrMeasurements > O(M^2 B \log(1/\delta) \frac{1}{\epsilon^2})$ i.i.d. samples from $\DistInliers$. Then, with probability at least $1-\delta$, for ever $\vxx \in H$: (\LC{to be extended to vectors})
\begin{align}
\overbrace{ \Expect{\DistInliers}{ ( y - h(\vxx) )^2 } }^{ \trimmederr_{\DistInliers}(\vxx) }
 \leq 
\overbrace{ \aveOverMeas ( y_i - h_i(\vxx) )^2 }^{ \err_{\DistSampleInliers}(\vxx) } + \epsilon
\end{align}
proving the second claim in eq.~\eqref{eq:proof-claim2}.
\end{fact}
% --------
\end{proof}

%=================================================================
\subsubsection{Putting things together}

Now we mostly need to bound $\sqrt{ \Expect{\DistSampleInliers}{  \residual{\vxx\gt}^4 } } $

\LC{we can directly cite the following:}
\grayout{
\begin{lemma}[Lemma 5.5 in~\cite{Klivans18arxiv-robustRegression}]
\label{lem:clippingDists}
For every distribution $\DistInliers$ on $\Real{\dimAmbient} \times [-M,M]^\dimy$ such that $e_4 = \Expect{\DistInliers}{  \residual{\vxx\gt}^4 } < \infty$, there exists a distribution $\calF$ such that $\normTV{\DistInliers - \calF} \leq \outlierRate$ and $\residual{\vxx\gt}^4$ is bounded absolutely in the support of $\calF$ 
by $e_4 / \outlierRate$.
\end{lemma}

\begin{proof}
Set $\calF \doteq \DistInliers \;|\; \left\{ \residual{\vxx\gt}^4  \leq e_4  / \outlierRate \right\}$. Then, by definition $\calF$ is bounded by $e_4 / \outlierRate$. 
\LC{ Furthermore, by Markov's inequality, the probability of $\left\{ \residual{\vxx\gt}^4 \leq e_4  / \outlierRate \right\}$ is at least $1-\outlierRate$, concluding the proof.}
\end{proof}

\begin{proof}[Proof of \cref{thm:lowOut-apriori-LTS}] \LC{to revisit with Gaussian assumption}
Let $e_4 = \Expect{\DistInliers}{  \residual{\vxx\gt}^4 }$. Without loss of generality, by using 
\cref{lem:clippingDists}, we can assume that $\residual{\vxx\gt}^4$ is bounded above by $e_4/\outlierRate$ in $\DistInliers$. 
\LC{Using Hoeffding's inequality, if $\nrMeasurements \geq e_4 \frac{\log(1/\delta)}{\outlierRate \epsilon^2}$, then with probability at least $1-\delta$, $\Expect{\DistSampleInliers}{  \residual{\vxx\gt}^4 } \leq 
\Expect{\DistInliers}{  \residual{\vxx\gt}^4 } + \epsilon$.}
By~\cref{lem:boundingOptError} and~\cref{lem:boundingGenError} and the inequality above, with probability $1-O(\epsilon)$,
\begin{align}
\trimmederr_\DistInliers( \vxx\ltssdp ) \leq  
(1 + O(\kappa) \outlierRate^{1 - \frac{2}{k}}  ) \optt_{\DistInliers,B}
+
O(\kappa) \outlierRate^{1 - \frac{2}{k}}  \sqrt{ \Expect{\DistInliers}{  \residual{\vxx\gt}^4 } } + O(\kappa\epsilon)
\end{align}
from which \cref{thm:lowOut-apriori-LTS} follows by choosing $\epsilon$ to be a sufficiently small constant time the parameter desired.
\end{proof}
}

==> lts-discarded-notation.tex <==

$\opttsos^{\frac{k}{2}} = \scenario{optimal\_objective\_relaxation}~\eqref{eq:lts1}$

Let
$\DistInliers$: true inlier distribution.
$\DistSampleInliers$: uniform distribution over sampled inliers.

\begin{align}
\label{eq:errorAtx}
\err_\DistInliers(\vxx) = \Expect{ \DistInliers }{ \residual{\vxx}^2  }
\end{align}

% \begin{align}
% \label{eq:errorAtx}
% \trimmederr_\DistInliers(\vxx) = \Expect{ \DistInliers }{ \normTwo{\vy - \trim_M(\MA\tran \vxx) }^2  }
% \end{align}
% where $\trim_M$ clips the entries of a vector between $[-M,M]$.

%For a real random variable $a \in \Real{}$, $\normk{a} = \Expect{}{a^k}^{\frac{1}{k}}$.

\begin{itemize}
\item $\InlierSet$: set of indices (with $\InlierSet \subseteq [\nrMeasurements]$) corresponding to the inlier measurements;
\item $\DistInliers$: distribution producing the matrices $\MA_i$, $i\in[\nrMeasurements]$ for the inlier measurements;
\item $\DistSampleInliers$: uniform distribution over the set $\MA_i$, $i\in[\nrMeasurements]$. 
\end{itemize}
